Fair admission risk prediction with proportional multicalibration

Fair calibration is a widely desirable fairness criteria in risk prediction contexts. One way to measure and achieve fair calibration is with multicalibration. Multicalibration constrains calibration error among flexibly-defined subpopulations while maintaining overall calibration. However, multicalibrated models can exhibit a higher percent calibration error among groups with lower base rates than groups with higher base rates. As a result, it is possible for a decision-maker to learn to trust or distrust model predictions for specific groups. To alleviate this, we propose \emph{proportional multicalibration}, a criteria that constrains the percent calibration error among groups and within prediction bins. We prove that satisfying proportional multicalibration bounds a model's multicalibration as well its \emph{differential calibration}, a fairness criteria that directly measures how closely a model approximates sufficiency. Therefore, proportionally calibrated models limit the ability of decision makers to distinguish between model performance on different patient groups, which may make the models more trustworthy in practice. We provide an efficient algorithm for post-processing risk prediction models for proportional multicalibration and evaluate it empirically. We conduct simulation studies and investigate a real-world application of PMC-postprocessing to prediction of emergency department patient admissions. We observe that proportional multicalibration is a promising criteria for controlling simultaneous measures of calibration fairness of a model over intersectional groups with virtually no cost in terms of classification performance.

==> tbls/fairness_metrics.tex <==
\begin{table}[b]
    % \begin{tabularx}[0.5\textwidth]{
    % \end{tabularx}
    \scriptsize
    \caption{
        ML definitions of fairness, based the distributions of model predictions ($\mathcal{R}$), demographics ($A$), and data labels ($Y$). 
        Adapted from~\textcite{barocasFairnessMachineLearning}. 
    }\label{tbl:fairness_metrics}
    % \rowcolors{2}{white}{gray!15}
    \begin{tabularx}{ \textwidth }{ l l X X}
        \toprule
        Measure     &   Definition      &   Meaning     &   Use Case and Assumptions   \\
        \midrule
        Demographic Parity      &   $ \Yhat \perp A $     
                                &   Model's predictions should be independent of patient demographics.    
                                &   Useful if a subset of patients is expected to be under-diagnosed in the data.
                                    Assumes predictions ought to be equally distributed across demographic groups. 
                                \\
        Equalized Odds          &   $ \Yhat \perp A | Y $
                                &   For a given outcome, model's predictions should be independent of patient demographics.  
                                &   Equalizes the FP and FN rates of the model's predictions across demographic groups.  
                                    Allows prevalence of the outcome to differ demographically.                                \\
        Equalized Calibration   &   $ Y \perp A | \Yhat $
                                &   Model's risk predictions should reflect actual population risk, regardless of patient demographics.  
                                &   Useful when model predictions are interpreted as probabilities of the outcome occuring. 
                                    Guarantees that patients can be fairly ranked by risk score. 
        \\ 
        \bottomrule
    \end{tabularx}
\end{table}

